TFDM: Time-Variant Frequency-Based Point Cloud Diffusion with Mamba

Diffusion models currently demonstrate impressive performance over various generative tasks. Recent work on image diffusion highlights the strong capabilities of Mamba (state space models) due to its efficient handling of long-range dependencies and sequential data modeling. Unfortunately, joint consideration of state space models with 3D point cloud generation remains limited. To harness the powerful capabilities of the Mamba model for 3D point cloud generation, we propose a novel diffusion framework containing dual latent Mamba block (DM-Block) and a time-variant frequency encoder (TF-Encoder). The DM-Block apply a space-filling curve to reorder points into sequences suitable for Mamba state-space modeling, while operating in a latent space to mitigate the computational overhead that arises from direct 3D data processing. Meanwhile, the TF-Encoder takes advantage of the ability of the diffusion model to refine fine details in later recovery stages by prioritizing key points within the U-Net architecture. This frequency-based mechanism ensures enhanced detail quality in the final stages of generation. Experimental results on the ShapeNet-v2 dataset demonstrate that our method achieves state-of-the-art performance (ShapeNet-v2: 0.14\% on 1-NNA-Abs50 EMD and 57.90\% on COV EMD) on certain metrics for specific categories while reducing computational parameters and inference time by up to 10$\times$ and 9$\times$, respectively. Source code is available in Supplementary Materials and will be released upon accpetance.

==> sec/3_preliminary.tex <==
\section{Preliminary}
\label{sec:pre}

We present a range of required prerequisites to our method.

\begin{figure*}[hbt!]
\begin{center}
\includegraphics[width=1.0\linewidth]{Figures/FIgure3.pdf} 
% \framebox(450,150){}
\end{center}
   \vspace{-6mm}
   \caption{Qualitative results compare with other works. Three categories are illustrated here.}
   % \vspace{-5mm}
\label{fig:overview}
\end{figure*}


\subsection{Denoising Diffusion Probabilistic Model}
\label{sec:3.1}
For given samples $x_0\sim q(x_{0})$, the diffusion model gradually reverses a Markovian fixed forward diffusion process:
\begin{align}
    q(\mathbf{x}_{1:T}|\mathbf{x}_0)&= \prod\nolimits_{t=1}^{T} q(\mathbf{x}_{t}|\mathbf{x}_{t-1}),\\
    q(\mathbf{x}_{t}|\mathbf{x}_{t-1}) &=\mathcal{N}({\mathbf{x}_{t}; \sqrt{\alpha_{t}}\mathbf{x}_{t-1}, (1-\alpha_{t})\mathbf{I}}),
\end{align}
where $T$ denotes the time step, $q(\mathbf{x}_{t}|\mathbf{x}_{t-1})$ is the transition kernel progressively perturbs the input with a sequence of pre-defined variance schedule $(1-\alpha_{1}),...,(1-\alpha_{T})$. 

The reverse process is parameterized as a Markovian chain $p_{\theta}(\mathbf{x}_{0:T})$ which is equal to $p(\mathbf{x}_{T})\prod\nolimits_{t=1}^{T} p_{\theta}(\mathbf{x}_{t-1}|\mathbf{x}_{t})$,
\begin{equation}
    p_{\theta}(\mathbf{x}_{t-1}|\mathbf{x}_{t}) = \mathcal{N}(\mathbf{x}_{t-1};{\mu}_\theta(\mathbf{x}_t,t),\sigma_t^2\mathbf{I}),
    \label{model_obj}
\end{equation}
where $p(\mathbf{x}_T)$ is standard Gaussian and ${\mu}_\theta(\mathbf{x}_t,t)$ is the learnable object, with setting $\sigma_t^2$ as a fixed variance schedule.  This object is optimized by matching the ground truth denoising step, which can be interpreted as learning the source noise  ${\epsilon}_0$ by minimizing $w\left(t\right)\parallel{{\mathbf{\epsilon}}}_\theta\left(x_t,t\right)-{\epsilon}_0\parallel_2^2$, where $w\left(t\right)$ is a parameter only depends on timestep. The optimization objective thus becomes:
\begin{equation}
    \mathcal{L} = \mathbb{E}_{t\sim [1,T]}w\left(t\right)\parallel{{\mathbf{\epsilon}}}_\theta\left(\mathbf{x}_{t},t\right)-{\epsilon}_0\parallel_2^2
    \label{loss}
\end{equation}
After training, generation can be achieved via the inverse chain by sampling from a standard Gaussian distribution.


\subsection{State Space Model}
\label{sec:3.2}
The State Space Model (SSM)~\cite{mamba_initial} can be described as a continuous system that maps a 1-D function or sequence $x(t)$ to $y(t)$ , with medilated through a N-D latent state $h(t)$.
\begin{equation}
    h^{'}(t) = \mathbf{A}h(t) + \mathbf{B}x(t), y(t) = \mathbf{C}h(t), 
\end{equation}
where $\mathbf{A},\mathbf{B}$ and $\mathbf{C}$ are parameters can be learned via gradient descent. 
Mamba~\cite{mamba_initial} improved the SSM by relaxing the time-invariance constraint and discretize the formulation via a timescable transformation parameter $\Delta$. By using zero-order hold techniques, the parameters can be defined as:
\begin{equation} 
  \label{eq:mamba}
  \overline{\mathbf{A}} = \exp(\Delta \mathbf{A}), \overline{\mathbf{B}} = (\Delta \mathbf{A})^{-1} \left( \exp(\Delta \mathbf{A}) - \mathbf{I} \right) \Delta \mathbf{B} 
\end{equation}
Subsequently, \cref{eq:mamba} can be discretized and is able to compute the outputs as specific time step: 
\begin{equation}
    h^{'}(t) = \overline{\mathbf{A}}h(t) + \overline{\mathbf{C}}x(t), y(t) = \mathbf{C}h(t) 
\end{equation}
Finally, it employs a structured global convolution to enhance computational efficiency:
\begin{equation} 
   \overline{\mathbf{K}} = (\mathbf{C}\overline{\mathbf{B}},\ \mathbf{C}\overline{\mathbf{A}\mathbf{B}},\ \ldots,\ \mathbf{C}\overline{\mathbf{A}}^{M-1}\overline{\mathbf{B}}), \quad y = x * \overline{\mathbf{K}}, 
\end{equation}
where $M$ and $\overline{\mathbf{K}}$ represent individually the length of sequence x and the kernel of the global convolution.


\subsection{Graph Filter}
\label{sec:3.3}
Given a graph $\mathcal{G} = (\mathcal{V},\mathbf{A},\mathbf{A}^u)$ let $\mathcal{V}= { v_1,...,v_N }$ denote a set of $N$ nodes and $\mathbf{A},\mathbf{A}^u \in \mathbb{R}^{N\times N}$ represent the weight and unweight adjacency matrix. We refer to one-channel features on all nodes to be a graph signal $\mathbf{s}\in \mathbb{R}^N$. $\mathbf{A}$ has eigen decomposition $\mathbf{A}=V\mathbf{\Lambda}V^{-1}$ where the matrix $V$
contains eigenvectors of $\mathbf{A}$ and $\mathbf{\Lambda}$ is diagonal eigenvalue matrix corresponding to ordered eigenvalues $\lambda_1,...,\lambda_N$. 

As stated in~\cite{garph_signal}, the ordered eigenvalues represent frequencies on the graph. Consider $\mathbf{A}$ as a graph shift operator and take a signal $\mathbf{s}$ to produce $\mathbf{y}= \mathbf{As}$, which is $V^{-1}\mathbf{y}=\mathbf{\Lambda}V^{-1}\mathbf{s} $. The graph Fourier transformation of graph signal $\mathbf{s}$ and $ \mathbf{y}$ :  $ \mathbf{\hat{s}}= V^{-1}\mathbf{s} ,\mathbf{\hat{y}}= V^{-1}\mathbf{y}$ could be considered as frequency contents of signal $\mathbf{s}$ and $\mathbf{y}$. Additionally, a graph filter is a polynomial in the graph shift~\cite{graph_signal2}: $h(\mathbf{A})=\sum_{l=0}^{L-1} h_{l}\mathbf{A}^l$, where 
$h_{l}, L $ denote filter coefficients and the length of filter respectively. This filter takes signal $\mathbf{s}$ and generate $\mathbf{y}=h(\mathbf{A})\mathbf{s} = Vh(\mathbf{\Lambda}V^{-1}\mathbf{s})$, making $V^{-1}\mathbf{y}=h(\mathbf{\Lambda}V^{-1}\mathbf{s})$ then $\mathbf{\hat{y}} =h(\mathbf{\Lambda} \mathbf{\hat{s}})$. The diagonal matrix $h(\mathbf{\Lambda})$ is the graph frequency response of the filter
$h(\mathbf{A})$ can be denoted $\hat{h}(\mathbf{A})$, and the frequency response of $\lambda_{i}$ is $\sum_{l=1}^{L-1}h_{l}\lambda_{i}^l$.


